Matrix-free construction of HSS representation using adaptive randomized sampling

We present new algorithms for the randomized construction of hierarchically semi-separable matrices, addressing several practical issues. The HSS construction algorithms use a partially matrix-free, adaptive randomized projection scheme to determine the maximum off-diagonal block rank. We develop both relative and absolute stopping criteria to determine the minimum dimension of the random projection matrix that is sufficient for the desired accuracy. Two strategies are discussed to adaptively enlarge the random sample matrix: repeated doubling of the number of random vectors, and iteratively incrementing the number of random vectors by a fixed number. The relative and absolute stopping criteria are based on probabilistic bounds for the Frobenius norm of the random projection of the Hankel blocks of the input matrix. We discuss parallel implementation and computation and communication cost of both variants. Parallel numerical results for a range of applications, including boundary element method matrices and quantum chemistry Toeplitz matrices, show the effectiveness, scalability and numerical robustness of the proposed algorithms.

==> tex/algo/adaptive_comp_node_update.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Updated Adaptive Node Compression

%\begin{algorithm}[!ht]
\begin{algorithm}[p]
  \DontPrintSemicolon
  \SetAlgoLined
  \SetKwProg{Fn}{function}{}{}
  \SetKwFunction{compressadaptive}{HSSCompressAdaptive}
  \SetKwFunction{compressnodeadaptive}{CompressNodeAdaptive}
  \SetKwFunction{compresssync}{CompressNodesSync}
  \SetKwFunction{root}{root}
  \SetKwFunction{randn}{randn}
  \SetKwFunction{min}{min}
  \SetKwData{synced}{sync}
  \SetKwData{COMPRESSED}{COMPRESSED}
  \SetKwData{UNTOUCHED}{UNTOUCHED}
  \SetKwData{state}{state}
  \SetKwData{Ustate}{Ustate}
  \SetKwData{Vstate}{Vstate}
  \Fn{$H =$ \compressadaptive{$A$, $\mathcal{T}$, $\varepsilon$, $d_0$, $\Delta d$}}{
    $d \gets d_0$ \\
    $R \gets $ \randn{$N, d$} \\
    $S^r \gets AR$ \\
    $S^c \gets A^*R$ \\
    \lForEach{$\tau \in \mathcal{T}$}{$\tau.\Ustate \gets \tau.\Vstate \gets \UNTOUCHED$}
    \While{\root{$\mathcal{T}$}$.\Ustate \neq \COMPRESSED$ {\bf and} $d < d_{\text{max}}$}{
      $\bar{R} \gets$ \randn{$N$, $\Delta d$} \\
      $R \gets \begin{bmatrix} R & \bar{R} \end{bmatrix}$ \\
      $S^r \gets \begin{bmatrix} S^r & A \bar{R} \end{bmatrix}$ \\
      $S^c \gets \begin{bmatrix} S^r & A^* \bar{R} \end{bmatrix}$ \\
      \compressnodeadaptive{$A$, $R$, $S^r$, $S^c$, \root{$\mathcal{T}$}, $\varepsilon$, $d$, $\Delta d$}\\
      $d \gets d + \Delta d$ \\
    }
    \Return $\mathcal{T}$
  }
  \caption{\emph{Adaptive} HSS compression of
  $A \in \mathbb{R}^{N \times N}$ with tolerance $\varepsilon$,
  partition tree $\mathcal{T}$. }
  \label{algo::AdaptiveHSScompress}
\end{algorithm}


\begin{algorithm}[!ht]
  \DontPrintSemicolon
  \SetAlgoLined
  \SetKwProg{Fn}{function}{}{end}
  \SetKwFunction{compressnodeadaptive}{CompressNodeAdaptive}
  \SetKwFunction{extract}{ExtractElements}
  \SetKwFunction{localsamples}{ComputeLocalSamples}
  \SetKwFunction{reducelocalsamples}{ReduceLocalSamples}
  \SetKwFunction{isleaf}{isleaf}
  \SetKwFunction{isroot}{isroot}
  \SetKwFunction{child}{children}
  \SetKwFunction{ID}{ID}
  \SetKwFunction{max}{max}
  \SetKwFunction{cols}{cols}
  \SetKwFunction{rows}{rows}
  \SetKwFunction{QR}{QR}
  \SetKwData{UNTOUCHED}{UNTOUCHED}
  \SetKwData{COMPRESSED}{COMPRESSED}
  \SetKwData{PARTIALLYCOMPRESSED}{PARTIALLY\_COMPRESSED}
  \SetKwData{state}{state}
  \SetKwData{Ustate}{Ustate}
  \SetKwData{Vstate}{Vstate}

  \Fn{\compressnodeadaptive{$A$, $R$, $S^r$, $S^c$, $\tau$, $\varepsilon$, $d$, $\Delta d$}} {
    \uIf{\isleaf{$\tau$}}{
      \uIf{$\tau.\Ustate = \UNTOUCHED$ {\bf and} $\tau.\Vstate = \UNTOUCHED$}{
        $\tau.D \gets$ \extract{$A$, $\tau.I$, $\tau.I$}}
    }
    \uElse{
      $\nu_1, \nu_2 \gets$ \child{$\tau$} \\
      \compressnodeadaptive{$A$, $R$, $S^r$, $S^c$, $\nu_1$, $\varepsilon$, $d$, $\Delta d$}\\
      \compressnodeadaptive{$A$, $R$, $S^r$, $S^c$, $\nu_2$, $\varepsilon$, $d$, $\Delta d$}\\
      \lIf{$\nu_1.\Ustate \neq \COMPRESSED$ {\bf or} $\nu_1.\Vstate \neq \COMPRESSED$}{\Return}
      \lIf{$\nu_2.\Ustate \neq \COMPRESSED$ {\bf or} $\nu_2.\Vstate \neq \COMPRESSED$}{\Return}
      \uIf{$\tau.\Ustate = \UNTOUCHED$ {\bf and} $\tau.\Vstate = \UNTOUCHED$}{
        $\tau.B_{12} \gets$ \extract{$A$, $\nu_1.I^r$, $\nu_2.I^c$} \\
        $\tau.B_{21} \gets$ \extract{$A$, $\nu_2.I^r$, $\nu_1.I^c$}
      }
    }
    \uIf{\isroot{$\tau$}}{
      $\tau.\Ustate \gets \tau.\Vstate \gets \COMPRESSED$ \\
      \Return
    }
    \lIf{$\tau.\Ustate = \UNTOUCHED$}{
      \localsamples{$R$, $S^r$, $S^c$, $\tau$, $1: (d+\Delta d)$} %\tcp*[f]{Compute all $d$ columns of $\tau.S^{r/c}$ \& $\tau.R^{r/c}$}
    }\lElse{
      \localsamples{$R$, $S^r$, $S^c$, $\tau$, $d : (d+\Delta d)$} %\tcp*[f]{Only last $\Delta d$ columns}
    }
    \uIf{$\tau.\Ustate \neq \COMPRESSED$ {\bf or} $\tau.\Vstate \neq \COMPRESSED$} {
      \uIf{$\tau.\Ustate = \UNTOUCHED$ {\bf or} $\tau.\Vstate = \UNTOUCHED$}{
        $i_1 \gets \emptyset$\\
        $i_2 \gets 1:d$\\
      }\uElse{
        $i_1 \gets 1:(d-\Delta d)$\\
        $i_2 \gets (d-\Delta d+1):d$\\
      }
      $i_3 \gets (d+1):(d+\Delta d)$\\
      Notation, let $Q_{i} \equiv \tau.Q(:, i)$ and $S_{i} \equiv \tau.S(:, i)$ \\
      \uIf{$\tau.\Ustate \neq \COMPRESSED$}{
        $Q^r_{i_2} \gets $ \QR{$Q^r_{i_2}$} \hfill \tcp*[h]{Orthogonalization}\\
        $Q^r_{i_3} \gets S^r_{i_3} - Q^r_{i_1 \cup i_2} \left(Q^r_{i_1 \cup i_2}\right)^* S^r_{i_3} $\\
        \uIf{$\|Q^r_{i_3}\| < \varepsilon / \left(10 \sqrt{\frac{2}{\pi}} \right)$}{
          $\{ (\tau.U)^*,\,\, \tau.J^r \} \gets $ \ID{$\left(S^r_{i_1 \cup i_2}\right)^*, \varepsilon$}\\
          $\tau.\Ustate \gets \COMPRESSED$ \\
        }\lElse{$\tau.\Ustate \gets \PARTIALLYCOMPRESSED$}
      }
      \uIf{$\tau.\Vstate \neq \COMPRESSED$}{
        $Q^c_{i_2} \gets $ \QR{$Q^c_{i_2}$} \\
        $Q^c_{i_3} \gets S^c_{i_3} - Q^c_{i_1 \cup i_2} \left( Q^c_{i_1 \cup i_2}\right)^* S^c_{i_3} $\\
        \uIf{$\|Q^c_{i_3}\| < \varepsilon / \left(10 \sqrt{\frac{2}{\pi}} \right)$}{
          $\{ (\tau.V)^*,\,\, \tau.J^c \} \gets $ \ID{$\left(S^c_{i_1 \cup i_2}\right)^*, \varepsilon$}\\
          $\tau.\Vstate \gets \COMPRESSED$ \\
        }\lElse{$\tau.\Vstate \gets \PARTIALLYCOMPRESSED$}
      }
      \uIf{$\tau.\Ustate = \COMPRESSED$ {\bf and} $\tau.\Vstate = \COMPRESSED$}{
        \reducelocalsamples{$R$, $\tau$, $1:(d+\Delta d)$} %\tcp*[f]{Update all $d$ columns of $\tau.S^{r/c}$ \& $\tau.R^{r/c}$}
      }
    }
    \lElse{\reducelocalsamples{$R$, $\tau$, $d: (d+\Delta d)$}}

  }
  \caption{Adaptive recursive compression of an HSS node $\tau$ of a
    matrix $A$ with tolerance $\varepsilon$ using the random matrix
    $R$ and the random samples $S^r$ and $S^c$ ($d$ vectors, with
    $\Delta d$ new ones to check quality of the first $d$ vectors).}
  \label{algo::HSScompressNodeAdaptive}
\end{algorithm}





















\begin{algorithm}[!ht]
  \DontPrintSemicolon
  \SetAlgoLined
  \SetKwProg{Fn}{function}{}{}
  \SetKwFunction{localsamples}{ComputeLocalSamples}
  \SetKwFunction{isleaf}{isleaf}
  \SetKwFunction{cols}{columns}
  \SetKwFunction{child}{children}
  \SetKwFunction{reducelocalsamples}{ReduceLocalSamples}

  \Fn{\localsamples{$R$, $S^r$, $S^c$, $\tau$, $i$}} {
    % $i \gets a : b$ \tcp*[f]{Index set of only the last $\Delta d$ columns} \\
    \uIf{\isleaf{$\tau$}}{
      $\tau.S^r(\,:\,,i) \gets S^r(\tau.I,i) - \tau.D \,\, R(\tau.I,i)$ \\
      $\tau.S^c(\,:\,,i) \gets S^c(\tau.I,i) - (\tau.D)^* \,\, R(\tau.I,i)$ \\
    }\Else{
      $\nu_1, \nu_2 \gets$ \child{$\tau$} \\
      $\tau.S^r(\,:\,,i) \gets \begin{bmatrix} \nu_1.S^r(\nu_1.J^r,i) - \tau.B_{12} \,\, \nu_2.R^r \\
        \nu_2.S^r(\nu_2.J^r,i) - \tau.B_{21} \,\, \nu_1.R^r \end{bmatrix}$ \\
      $\tau.S^c(\,:\,,i) \gets \begin{bmatrix} \nu_1.S^c(\nu_1.J^c,i) - (\tau.B_{21})^* \,\, \nu_2.R^c \\
        \nu_2.S^c(\nu_c.J^c,i) - (\tau.B_{12})^* \,\, \nu_1.R^c \end{bmatrix}$ \\
    }
  }
  \BlankLine
  \Fn{\reducelocalsamples{$R$, $\tau$, $i$}}{
    % $\tau.S^r(\,:\,,i) \gets \tau.S^r(\tau.J^r, i)$ \\
    % $\tau.S^c(\,:\,,i) \gets \tau.S^c(\tau.J^c, i)$ \\
    \uIf{\isleaf{$\tau$}}{
      $\tau.R^r \gets (\tau.V)^* \,\, R(\tau.I,i)$ \\
      $\tau.R^c \gets (\tau.U)^* \,\, R(\tau.I,i)$ \\
      $\tau.I^r \gets \tau.I(\tau.J^r)$ \\
      $\tau.I^c \gets \tau.I(\tau.J^c)$
    }\Else{
      $\nu_1, \nu_2 \gets$ \child{$\tau$} \\
      $\tau.R^r \gets (\tau.V)^* \begin{bmatrix} \nu_1.R^r \\ \nu_2.R^r \end{bmatrix}$ \\
      $\tau.R^c \gets (\tau.U)^* \begin{bmatrix} \nu_1.R^c \\ \nu_2.R^c \end{bmatrix}$ \\
      $\tau.I^r \gets \begin{bmatrix} \nu_1.I^r & \nu_2.I^r \end{bmatrix}(\tau.J^r)$ \\
      $\tau.I^c \gets \begin{bmatrix} \nu_1.I^c & \nu_2.I^c \end{bmatrix}(\tau.J^c)$
    }
  }
  \caption{Compute local samples and reduce local samples based on
    rows selected by the interpolative decomposition.}
  \label{algo::computelocalsamples}
\end{algorithm}



==> tex/algo/comp_local_reduce.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Compute Local Samples and Reduce Local Samples

\begin{algorithm2e}  %[!ht]
%\begin{algorithm}[p]
  \DontPrintSemicolon
  \SetAlgoLined
  \SetKwProg{Fn}{function}{}{}
  \SetKwFunction{localsamples}{ComputeLocalSamples}
  \SetKwFunction{isleaf}{isleaf}
  \SetKwFunction{cols}{columns}
  \SetKwFunction{child}{children}
  \SetKwFunction{reducelocalsamples}{ReduceLocalSamples}

  \Fn{\localsamples{$R$, $S^r$, $S^c$, $\tau$, $d \gets \cols{R}$, $\Delta d \gets d$}} {
    $\bar{d} \gets (d-\Delta d) : d$ \tcp*[f]{Index set of only the last $\Delta d$ columns} \\
    \uIf{\isleaf{$\tau$}}{
      $\tau.S^r(\,:\,,\bar{d}) \gets S^r(\tau.I,\bar{d}) - \tau.D \,\, R(\tau.I,\bar{d})$ \\
      $\tau.S^c(\,:\,,\bar{d}) \gets S^c(\tau.I,\bar{d}) - (\tau.D)^* \,\, R(\tau.I,\bar{d})$ \\
    }
    \Else{
      $\nu_1, \nu_2 \gets$ \child{$\tau$} \\
      $\tau.S^r(\,:\,,\bar{d}) \gets \begin{bmatrix} \nu_1.S^r(\nu_1.J^r,\bar{d}) - \tau.B_{12} \,\, \nu_2.R^r \\
        \nu_2.S^r(\nu_2.J^r,\bar{d}) - \tau.B_{21} \,\, \nu_1.R^r \end{bmatrix}$ \\
      $\tau.S^c(\,:\,,\bar{d}) \gets \begin{bmatrix} \nu_1.S^c(\nu_1.J^c,\bar{d}) - (\tau.B_{21})^* \,\, \nu_2.R^c \\
        \nu_2.S^c(\nu_c.J^c,\bar{d}) - (\tau.B_{12})^* \,\, \nu_1.R^c \end{bmatrix}$ \\
    }
  }
  \BlankLine
  \Fn{\reducelocalsamples{$R$, $\tau$, $d \gets \cols{R}$, $\Delta d \gets d$}}{
    % $\tau.S^r(\,:\,,\bar{d}) \gets \tau.S^r(\tau.J^r, \bar{d})$ \\
    % $\tau.S^c(\,:\,,\bar{d}) \gets \tau.S^c(\tau.J^c, \bar{d})$ \\
    \uIf{\isleaf{$\tau$}}{
      $\tau.R^r \gets (\tau.V)^* \,\, R(\tau.I,\bar{d})$ \\
      $\tau.R^c \gets (\tau.U)^* \,\, R(\tau.I,\bar{d})$ \\
      $\tau.I^r \gets \tau.I(\tau.J^r)$ \\
      $\tau.I^c \gets \tau.I(\tau.J^c)$
    }
    \Else{
      $\nu_1, \nu_2 \gets$ \child{$\tau$} \\
      $\tau.R^r \gets (\tau.V)^* \begin{bmatrix} \nu_1.R^r \\ \nu_2.R^r \end{bmatrix}$ \\
      $\tau.R^c \gets (\tau.U)^* \begin{bmatrix} \nu_1.R^c \\ \nu_2.R^c \end{bmatrix}$ \\
      $\tau.I^r \gets \begin{bmatrix} \nu_1.I^r & \nu_2.I^r \end{bmatrix}(\tau.J^r)$ \\
      $\tau.I^c \gets \begin{bmatrix} \nu_1.I^c & \nu_2.I^c \end{bmatrix}(\tau.J^c)$
    }
  }
  \caption{Compute local samples and reduce local samples based on
    rows selected by the interpolative decomposition. The total number
    of columns in $R$, $S^r$ and $S^c$ is $d$; $\Delta d$ columns
    where since the last restart.}
  \label{algo::computelocalsamples1}
\end{algorithm2e}



==> tex/algo/comp_node_adaptive_update.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Updated Adaptive Node Compression

%\begin{algorithm}[!ht]
\begin{algorithm}[p]
  \DontPrintSemicolon
  \SetAlgoLined
  \SetKwProg{Fn}{function}{}{end}
  \SetKwFunction{compressnodeadaptive}{CompressNodeAdaptive}
  \SetKwFunction{extract}{ExtractElements}
  \SetKwFunction{localsamples}{ComputeLocalSamples}
  \SetKwFunction{reducelocalsamples}{ReduceLocalSamples}
  \SetKwFunction{isleaf}{isleaf}
  \SetKwFunction{isroot}{isroot}
  \SetKwFunction{child}{children}
  \SetKwFunction{ID}{ID}
  \SetKwFunction{max}{max}
  \SetKwFunction{cols}{cols}
  \SetKwFunction{rows}{rows}
  \SetKwFunction{QR}{QR}
  \SetKwData{UNTOUCHED}{UNTOUCHED}
  \SetKwData{COMPRESSED}{COMPRESSED}
  \SetKwData{PARTIALLYCOMPRESSED}{PARTIALLY\_COMPRESSED}
  \SetKwData{state}{state}
  \SetKwData{Ustate}{Ustate}
  \SetKwData{Vstate}{Vstate}

  \Fn{\compressnodeadaptive{$A$, $R$, $S^r$, $S^c$, $\tau$, $\varepsilon$, $d$, $\Delta d$}} {
    \uIf{\isleaf{$\tau$}}{
      \uIf{$\tau.\Ustate = \UNTOUCHED$ {\bf and} $\tau.\Vstate = \UNTOUCHED$}{
        $\tau.D \gets$ \extract{$A$, $\tau.I$, $\tau.I$}}
    }
    \uElse{
      $\nu_1, \nu_2 \gets$ \child{$\tau$} \\
      \compressnodeadaptive{$A$, $R$, $S^r$, $S^c$, $\nu_1$, $\varepsilon$, $d$, $\Delta d$}\\
      \compressnodeadaptive{$A$, $R$, $S^r$, $S^c$, $\nu_2$, $\varepsilon$, $d$, $\Delta d$}\\
      \lIf{$\nu_1.\Ustate \neq \COMPRESSED$ {\bf or} $\nu_1.\Vstate \neq \COMPRESSED$}{\Return}
      \lIf{$\nu_2.\Ustate \neq \COMPRESSED$ {\bf or} $\nu_2.\Vstate \neq \COMPRESSED$}{\Return}
      \uIf{$\tau.\Ustate = \UNTOUCHED$ {\bf and} $\tau.\Vstate = \UNTOUCHED$}{
        $\tau.B_{12} \gets$ \extract{$A$, $\nu_1.I^r$, $\nu_2.I^c$} \\
        $\tau.B_{21} \gets$ \extract{$A$, $\nu_2.I^r$, $\nu_1.I^c$}
      }
    }
    \uIf{\isroot{$\tau$}}{
      $\tau.\Ustate \gets \tau.\Vstate \gets \COMPRESSED$ \\
      \Return
    }
    \lIf{$\tau.\state = \UNTOUCHED$}{
      \localsamples{$R$, $S^r$, $S^c$, $\tau$, $1: (d+\Delta d)$} %\tcp*[f]{Compute all $d$ columns of $\tau.S^{r/c}$ \& $\tau.R^{r/c}$}
    }\lElse{
      \localsamples{$R$, $S^r$, $S^c$, $\tau$, $d : (d+\Delta d)$} %\tcp*[f]{Only last $\Delta d$ columns}
    }
    \uIf{$\tau.\Ustate \neq \COMPRESSED$ {\bf or} $\tau.\Vstate \neq \COMPRESSED$} {
      \uIf{$\tau.\Ustate = \UNTOUCHED$ {\bf or} $\tau.\Vstate = \UNTOUCHED$}{
        $i_1 \gets \emptyset$\\
        $i_2 \gets 1:d$\\
      }\uElse{
        $i_1 \gets 1:(d-\Delta d)$\\
        $i_2 \gets (d-\Delta d+1):d$\\
      }
      $i_3 \gets (d+1):(d+\Delta d)$\\
      Notation, let $Q_{i} \equiv \tau.Q(:, i)$ and $S_{i} \equiv \tau.S(:, i)$ \\
      \uIf{$\tau.\Ustate \neq \COMPRESSED$}{
        $Q^r_{i_2} \gets $ \QR{$Q^r_{i_2}$} \hfill \tcp*[h]{Orthogonalization}\\
        $Q^r_{i_3} \gets S^r_{i_3} - Q^r_{i_1 \cup i_2} \left(Q^r_{i_1 \cup i_2}\right)^* S^r_{i_3} $\\
        \uIf{$\|Q^r_{i_3}\| < \varepsilon / \left(10 \sqrt{\frac{2}{\pi}} \right)$}{
          $\{ (\tau.U)^*,\,\, \tau.J^r \} \gets $ \ID{$\left(S^r_{i_1 \cup i_2}\right)^*, \varepsilon$}\\
          $\tau.\Ustate \gets \COMPRESSED$ \\
        }\lElse{$\tau.\Ustate \gets \PARTIALLYCOMPRESSED$}
      }
      \uIf{$\tau.\Vstate \neq \COMPRESSED$}{
        $Q^c_{i_2} \gets $ \QR{$Q^c_{i_2}$} \\
        $Q^c_{i_3} \gets S^c_{i_3} - Q^c_{i_1 \cup i_2} \left( Q^c_{i_1 \cup i_2}\right)^* S^c_{i_3} $\\
        \uIf{$\|Q^c_{i_3}\| < \varepsilon / \left(10 \sqrt{\frac{2}{\pi}} \right)$}{
          $\{ (\tau.V)^*,\,\, \tau.J^c \} \gets $ \ID{$\left(S^c_{i_1 \cup i_2}\right)^*, \varepsilon$}\\
          $\tau.\Vstate \gets \COMPRESSED$ \\
        }\lElse{$\tau.\Vstate \gets \PARTIALLYCOMPRESSED$}
      }
      \uIf{$\tau.\Ustate = \COMPRESSED$ {\bf and} $\tau.\Vstate = \COMPRESSED$}{
        \reducelocalsamples{$R$, $\tau$, $1:(d+\Delta d)$} %\tcp*[f]{Update all $d$ columns of $\tau.S^{r/c}$ \& $\tau.R^{r/c}$}
      }
    }
    \lElse{\reducelocalsamples{$R$, $\tau$, $d: (d+\Delta d)$}}

  }
  \caption{Adaptive recursive compression of an HSS node $\tau$ of a
    matrix $A$ with tolerance $\varepsilon$ using the random matrix
    $R$ and the random samples $S^r$ and $S^c$ ($d$ vectors, with
    $\Delta d$ new ones to check quality of the first $d$ vectors).}
  \label{algo::HSScompressNodeAdaptive}
\end{algorithm}


%\begin{algorithm}[!ht]
\begin{algorithm}[p]
  \DontPrintSemicolon
  \SetAlgoLined
  \SetKwProg{Fn}{function}{}{}
  \SetKwFunction{localsamples}{ComputeLocalSamples}
  \SetKwFunction{isleaf}{isleaf}
  \SetKwFunction{cols}{columns}
  \SetKwFunction{child}{children}
  \SetKwFunction{reducelocalsamples}{ReduceLocalSamples}

  \Fn{\localsamples{$R$, $S^r$, $S^c$, $\tau$, $i$}} {
    % $i \gets a : b$ \tcp*[f]{Index set of only the last $\Delta d$ columns} \\
    \uIf{\isleaf{$\tau$}}{
      $\tau.S^r(\,:\,,i) \gets S^r(\tau.I,i) - \tau.D \,\, R(\tau.I,i)$ \\
      $\tau.S^c(\,:\,,i) \gets S^c(\tau.I,i) - (\tau.D)^* \,\, R(\tau.I,i)$ \\
    }\Else{
      $\nu_1, \nu_2 \gets$ \child{$\tau$} \\
      $\tau.S^r(\,:\,,i) \gets \begin{bmatrix} \nu_1.S^r(\nu_1.J^r,i) - \tau.B_{12} \,\, \nu_2.R^r \\
        \nu_2.S^r(\nu_2.J^r,i) - \tau.B_{21} \,\, \nu_1.R^r \end{bmatrix}$ \\
      $\tau.S^c(\,:\,,i) \gets \begin{bmatrix} \nu_1.S^c(\nu_1.J^c,i) - (\tau.B_{21})^* \,\, \nu_2.R^c \\
        \nu_2.S^c(\nu_c.J^c,i) - (\tau.B_{12})^* \,\, \nu_1.R^c \end{bmatrix}$ \\
    }
  }
  \BlankLine
  \Fn{\reducelocalsamples{$R$, $\tau$, $i$}}{
    % $\tau.S^r(\,:\,,i) \gets \tau.S^r(\tau.J^r, i)$ \\
    % $\tau.S^c(\,:\,,i) \gets \tau.S^c(\tau.J^c, i)$ \\
    \uIf{\isleaf{$\tau$}}{
      $\tau.R^r \gets (\tau.V)^* \,\, R(\tau.I,i)$ \\
      $\tau.R^c \gets (\tau.U)^* \,\, R(\tau.I,i)$ \\
      $\tau.I^r \gets \tau.I(\tau.J^r)$ \\
      $\tau.I^c \gets \tau.I(\tau.J^c)$
    }\Else{
      $\nu_1, \nu_2 \gets$ \child{$\tau$} \\
      $\tau.R^r \gets (\tau.V)^* \begin{bmatrix} \nu_1.R^r \\ \nu_2.R^r \end{bmatrix}$ \\
      $\tau.R^c \gets (\tau.U)^* \begin{bmatrix} \nu_1.R^c \\ \nu_2.R^c \end{bmatrix}$ \\
      $\tau.I^r \gets \begin{bmatrix} \nu_1.I^r & \nu_2.I^r \end{bmatrix}(\tau.J^r)$ \\
      $\tau.I^c \gets \begin{bmatrix} \nu_1.I^c & \nu_2.I^c \end{bmatrix}(\tau.J^c)$
    }
  }
  \caption{Compute local samples and reduce local samples based on
    rows selected by the interpolative decomposition.}
  \label{algo::computelocalsamples2}
\end{algorithm}



==> tex/algo/comp_node_sync.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Adaptive HSS Node Compression with Sync

%\begin{algorithm}[!ht]
\begin{algorithm}[p]
  \DontPrintSemicolon
  \SetAlgoLined
  \SetKwProg{Fn}{function}{}{}
  \SetKwFunction{compresssync}{CompressNodesSync}
  \SetKwFunction{exchangeextractionindices}{ExchangeExtractionIndices}
  \SetKwFunction{extract}{ExtractElements}
  \SetKwFunction{localsamples}{ComputeLocalSamples}
  \SetKwFunction{reducelocalsamples}{ReduceLocalSamples}
  \SetKwFunction{isleaf}{isleaf}
  \SetKwFunction{isroot}{isroot}
  \SetKwFunction{child}{children}
  \SetKwFunction{ID}{ID}
  \SetKwFunction{levels}{levels}
  \SetKwFunction{level}{level}
  \SetKwFunction{local}{local}
  \SetKwFunction{allgather}{allgatherv}
  \SetKwBlock{Try}{try}{}
  \SetKwBlock{Fail}{catch}{}
  \SetKwData{UNTOUCHED}{UNTOUCHED}
  \SetKwData{COMPRESSED}{COMPRESSED}
  \SetKwData{PARTIALLYCOMPRESSED}{PARTIALLY\_COMPRESSED}
  \SetKwData{state}{state}

  \Fn{\compresssync{$A$, $R$, $S^r$, $S^c$, $\mathcal{T}$, $\varepsilon$, $d$, $\Delta d$}} {
    \For{$\ell =$ \levels{$\mathcal{T}$} {\bf to} $1$}{
      $\mathcal{J} \gets$ \exchangeextractionindices{$A$, $\mathcal{T}$, $\ell$} \\
      \ForEach{$\tau \in \mathcal{T}.$\level{$\ell$}}{
        \uIf{$\tau.\state = \UNTOUCHED$}{
          \uIf(\tcp*[f]{\underline{\emph{All processes}} participate in extraction of $\tau.D$}){\isleaf{$\tau$}}{
            \lIf{\local{$\tau$}}{$\tau.D \gets$ \extract{$A$, $\tau.I$, $\tau.I$}}
            \lElse{
              \extract{$A$, $\mathcal{J}.\tau.I$, $\mathcal{J}.\tau.I$} \tcp*[f]{Get $\tau.I$ from $\mathcal{J}$}
            }
          }
          \uElse(\tcp*[f]{\underline{\emph{All processes}} participate in extraction of $\tau.B_{12}$ and $\tau.B_{21}$}){
            $\nu_1, \nu_2 \gets$ \child{$\tau$} \\
            \uIf{$\nu_1.\state = \COMPRESSED$ {\bf and} $\nu_2.\state = \COMPRESSED$}{
              \uIf{\local{$\tau$}}{
                $\tau.B_{12} \gets$ \extract{$A$, $\nu_1.I^r$, $\nu_2.I^c$} \\
                $\tau.B_{21} \gets$ \extract{$A$, $\nu_2.I^r$, $\nu_1.I^c$}
              }\uElse{
                \extract{$A$, $\mathcal{J}.\nu_1.I^r$, $\mathcal{J}.\nu_2.I^c$} \\
                \extract{$A$, $\mathcal{J}.\nu_2.I^r$, $\mathcal{J}.\nu_1.I^c$}
              }
            }
          }
        }
      }
      \ForEach{$\tau \in \mathcal{T}.$\level{$\ell$}}{
        \lIf{$!$\local{$\tau$}}{\bf continue}
        \uIf{$!$\isleaf{$\tau$}}{
          \lIf{$\nu_1.\state \neq \COMPRESSED$ {\bf or} $\nu_2.\state \neq \COMPRESSED$)}{\bf continue}
        }
        \uIf{\isroot{$\tau$}}{
          $\tau.\state \gets \COMPRESSED$ \\
          \Return
        }
        \lIf{$\tau.\state = \UNTOUCHED$}{\localsamples{$R$, $S^r$, $S^c$, $\tau$}}
        \lElse{\localsamples{$R$, $S^r$, $S^c$, $\tau$, $d$, $\Delta d$}}
        \uIf{$\tau.\state \neq \COMPRESSED$}{
          \Try{
            $\{ (\tau.U)^*,\,\, \tau.J^r \} \gets$ \ID{$(\tau.S^r)^*$, $\varepsilon$} \\
            $\{ (\tau.V)^*,\,\, \tau.J^c \} \gets$ \ID{$(\tau.S^c)^*$, $\varepsilon$} \\
            $\tau.\state \gets \COMPRESSED$ \\
            \reducelocalsamples{$R$, $\tau$}
          }
          \Fail{
            $\tau.\state \gets \PARTIALLYCOMPRESSED$ \\
            \Return
          }
        }\lElse{\reducelocalsamples{$R$, $\tau$, $d$, $\Delta d$}}
      }
    }
  }
  \caption{Synchronized level-by-level (non-recursive) HSS compression
    of a matrix $A$ with tolerance $\varepsilon$, partition tree
    $\mathcal{T}$ and using random matrix $R$ and samples $S^r$ and
    $S^c$ ($d$ vectors, with $\Delta d$ new ones).}
  \label{algo::HSScompressNodeSync}
\end{algorithm}



==> tex/algo/exchange_indeces.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Exchange Indeces

%\begin{algorithm}[!ht]
\begin{algorithm}[p]
  \DontPrintSemicolon
  \SetAlgoLined
  \SetKwProg{Fn}{function}{}{}
  \SetKwFunction{exchangeextractionindices}{ExchangeExtractionIndices}
  \SetKwFunction{extract}{ExtractElements}
  \SetKwFunction{isleaf}{isleaf}
  \SetKwFunction{isroot}{isroot}
  \SetKwFunction{child}{children}
  \SetKwFunction{levels}{levels}
  \SetKwFunction{level}{level}
  \SetKwFunction{local}{local}
  \SetKwFunction{comm}{comm}
  \SetKwFunction{nrprocs}{nrprocs}
  \SetKwFunction{recv}{receive}
  \SetKwFunction{send}{send}
  \SetKwFunction{size}{size}
  \SetKwFunction{rank}{rank}
  \SetKwFunction{allgather}{allgatherv}
  \SetKwData{UNTOUCHED}{UNTOUCHED}
  \SetKwData{COMPRESSED}{COMPRESSED}
  \SetKwData{PARTIALLYCOMPRESSED}{PARTIALLY\_COMPRESSED}
  \SetKwData{state}{state}
  \SetKwData{dest}{dest}

  \Fn{$\mathcal{J} \gets$ \exchangeextractionindices{$\mathcal{T}$, $\ell$}}{
    \uIf{$\log{P} < 2^{\ell}-1$}{
      $\mathcal{J}_p \gets \emptyset$ \\
      \ForEach{$\tau \in \mathcal{T}.$\level{$\ell$}}{
        \uIf{\local{$\tau$} {\bf and} $\tau.\state = \UNTOUCHED$}{
          \lIf{\isleaf{$\tau$}}{
            $\mathcal{J}_p \gets \left\{ \mathcal{J}_p, \,\, \tau.I,\, \tau.I \right\}$
          }\uElse{
            $\nu_1, \nu_2 \gets$ \child{$\tau$} \\
            \uIf{$\nu_1.\state = \COMPRESSED$ {\bf and} $\nu_2.\state = \COMPRESSED$}{
              \lIf{\rank{$\nu_1.\comm$} $= 0$}{$\mathcal{J}_p \gets \left\{ \mathcal{J}_p, \,\, \nu_1.I^r,\, \nu_1.I^c \right\}$}
              \lIf{\rank{$\nu_2.\comm$} $= 0$}{$\mathcal{J}_p \gets \left\{ \mathcal{J}_p, \,\, \nu_2.I^r,\, \nu_2.I^c \right\}$}
            }
          }
        }
      }
      $\mathcal{J} \gets$ \allgather{$\mathcal{J}_p$}
    }\uElse{
      $\mathcal{J} \gets \emptyset$ \\
      \ForEach{$\tau \in \mathcal{T}.$\level{$\ell$}}{
        \uIf{$\tau.\state = \UNTOUCHED$}{
          \uIf{\local{$\tau$}}{
            \For{$p = 1$ {\bf to} $P$}{
              \uIf{$p \notin \tau.\comm$}{
                \uIf{$p \, \%$ \nrprocs{$\tau.\comm$} $=$ \rank{$\tau.\comm$}}{
                  \uIf{\isleaf{$\tau$}}{
                    \send{$p$, $\left\{ \tau.I , \tau.I \right\}$}
                  }\uElse{
                    $\nu_1, \nu_2 \gets$ \child{$\tau$} \\
                    \uIf{$\nu_1.\state = \COMPRESSED$ {\bf and} $\nu_2.\state = \COMPRESSED$}{
                      TODO must also send to sibling!! \\
                      \lIf{\rank{$\nu_1$} $= 0$}{\send{$p$, $\left\{ \nu_1.I^r, \nu_1.I^c \right\}$}}
                      \lIf{\rank{$\nu_2$} $= 0$}{\send{$p$, $\left\{ \nu_2.I^r, \nu_2.I^c \right\}$}}
                    }
                  }
                }
              }
            }
          }\lElse{$\mathcal{J} \gets \left\{ \mathcal{J}, \,\, \recv{} \right\}$}
        }
      }
    }
  }
  \caption{Exchange $\tau.I$, $\tau.I^r$, $\tau.I^c$, among all
    processes.}
  \label{algo::exchange_indices}
\end{algorithm}




==> tex/algo/hss_comp_adaptive.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Updated Adaptive Node Compression

\begin{algorithm2e}
  \DontPrintSemicolon
  \SetAlgoLined
  \SetKwProg{Fn}{function}{}{}
  \SetKwFunction{compressadaptive}{HSSCompressAdaptive}
  \SetKwFunction{compressnodeadaptive}{CompressNodeAdaptive}
  \SetKwFunction{compresssync}{CompressNodesSync}
  \SetKwFunction{root}{root}
  \SetKwFunction{randn}{randn}
  \SetKwFunction{min}{min}
  \SetKwData{synced}{sync}
  \SetKwData{COMPRESSED}{COMPRESSED}
  \SetKwData{UNTOUCHED}{UNTOUCHED}
  \SetKwData{state}{state}
  \SetKwData{Ustate}{Ustate}
  \SetKwData{Vstate}{Vstate}
  \Fn{$H =$ \compressadaptive{$A$, $\mathcal{T}$, $\varepsilon$, $d_0$, $\Delta d$}}{
    $d \gets d_0$ \\
    $R \gets $ \randn{$N, d$} \\
    $S^r \gets AR$ \\
    $S^c \gets A^*R$ \\
    \lForEach{$\tau \in \mathcal{T}$}{$\tau.\Ustate \gets \tau.\Vstate \gets \UNTOUCHED$}
    \While{\root{$\mathcal{T}$}$.\Ustate \neq \COMPRESSED$ {\bf and} $d < d_{\text{max}}$}{
      $\bar{R} \gets$ \randn{$N$, $\Delta d$} \\
      $R \gets \begin{bmatrix} R & \bar{R} \end{bmatrix}$ \\
      $S^r \gets \begin{bmatrix} S^r & A \bar{R} \end{bmatrix}$ \\
      $S^c \gets \begin{bmatrix} S^r & A^* \bar{R} \end{bmatrix}$ \\
      \compressnodeadaptive{$A$, $R$, $S^r$, $S^c$, \root{$\mathcal{T}$}, $\varepsilon$, $d$, $\Delta d$}\\
      $d \gets d + \Delta d$ \\
    }
    \Return $\mathcal{T}$
  }
  \caption{\emph{Adaptive} HSS compression of
  $A \in \mathbb{R}^{N \times N}$ with tolerance $\varepsilon$,
  partition tree $\mathcal{T}$. }
  \label{algo::AdaptiveHSScompress}
\end{algorithm2e}



==> tex/algo/hss_comp_adaptive_sync.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Adaptive HSS Compression

\begin{algorithm2e}
  \DontPrintSemicolon
  \SetAlgoLined
  \SetKwProg{Fn}{function}{}{}
  \SetKwFunction{compressadaptive}{HSSCompressAdaptive}
  \SetKwFunction{compressnodeadaptive}{CompressNodeAdaptive}
  \SetKwFunction{compresssync}{CompressNodesSync}
  \SetKwFunction{root}{root}
  \SetKwFunction{randn}{randn}
  \SetKwFunction{min}{min}
  \SetKwData{synced}{sync}
  \SetKwData{COMPRESSED}{COMPRESSED}
  \SetKwData{UNTOUCHED}{UNTOUCHED}
  \SetKwData{state}{state}

  \Fn{$H =$ \compressadaptive{$A$, $\mathcal{T}$, $\varepsilon$, \synced}}{
    $d \gets d_0$ \\
    $R \gets$ \randn{$N, d + \Delta d$} \\
    $S^r \gets A R$ \\
    $S^c \gets A^* R$ \\
    \lForEach{$\tau \in \mathcal{T}$}{$\tau.\state \gets \UNTOUCHED$}
    \lIf{\synced}{\compresssync{$A$, $R$, $S^r$, $S^c$, $\mathcal{T}$, $\varepsilon$, $d$, $0$}}
    \lElse{\compressnodeadaptive{$A$, $R$, $S^r$, $S^c$, \root{$\mathcal{T}$}, $\varepsilon$, $d$, $0$}}
    \While{\root{$\mathcal{T}$}$.\state \neq \COMPRESSED$ {\bf and} $d < d_{\text{max}}$}{
      \lIf{\synced}{\compresssync{$A$, $R$, $S^r$, $S^c$, $\mathcal{T}$, $\varepsilon$, $d$, $\Delta d$}}
      \lElse{\compressnodeadaptive{$A$, $R$, $S^r$, $S^c$, \root{$\mathcal{T}$}, $\varepsilon$, $d$, $\Delta d$}}
      $d \gets$ \min{$d + \Delta d$, $d_{\text{max}}$} \\
      $\bar{R} \gets$ \randn{$N$, $\Delta d$} \\
      $R \gets \begin{bmatrix} R & \bar{R} \end{bmatrix}$ \\
      $S^r \gets \begin{bmatrix} S^r & A \bar{R} \end{bmatrix}$ \\
      $S^c \gets \begin{bmatrix} S^r & A^* \bar{R} \end{bmatrix}$ \\
    }
    \Return $\mathcal{T}$
  }
  \caption{\emph{Adaptive} HSS compression of
    $A \in \mathbb{R}^{N \times N}$ with tolerance $\varepsilon$,
    partition tree $\mathcal{T}$ and synchronized element extraction
    if \texttt{sync = true}. }
  \label{algo::AdaptiveHSScompress_sync}
\end{algorithm2e}



==> tex/algo/hss_comp_node.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% HSS Compression Node Algorithm

% Note: This algorithm was commented out

%\begin{algorithm}[!ht]
\begin{algorithm}[p]
  \DontPrintSemicolon
  \SetAlgoLined
  \SetKwProg{Fn}{function}{}{}
  \SetKwFunction{compressnode}{CompressNode}
  \SetKwFunction{extract}{ExtractElements}
  \SetKwFunction{localsamples}{ComputeLocalSamples}
  \SetKwFunction{reducelocalsamples}{ReduceLocalSamples}
  \SetKwFunction{isleaf}{isleaf}
  \SetKwFunction{isroot}{isroot}
  \SetKwFunction{child}{children}
  \SetKwFunction{local}{local}
  \SetKwFunction{ID}{ID}

  \Fn{\compressnode{$A$, $R$, $S^r$, $S^c$, $\tau$, $\varepsilon$}} {
    \uIf{\isleaf{$\tau$}}{
      $\tau.D \gets$ \extract{$A$, $\tau.I$, $\tau.I$} \\
    }
    \uElse{
      $\nu_1, \nu_2 \gets$ \child{$\tau$} \\
      \lIf(\tcp*[f]{Recursion}){\local{$\nu_1$}}{\compressnode{$A$, $R$, $S^r$, $S^c$, $\nu_1$, $\varepsilon$}}
      \lIf{\local{$\nu_2$}}{\compressnode{$A$, $R$, $S^r$, $S^c$, $\nu_2$, $\varepsilon$}}
      $\tau.B_{12} \gets$ \extract{$A$, $\nu_1.I^r$, $\nu_2.I^c$} \\
      $\tau.B_{21} \gets$ \extract{$A$, $\nu_2.I^r$, $\nu_1.I^c$} \\
    }
    \lIf{\isroot{$\tau$}}{\Return}
    \localsamples{$R$, $S^r$, $S^c$, $\tau$} \\
    $\{ (\tau.U)^*,\,\, \tau.J^r \} \gets$ \ID{$(\tau.S^r)^*$, $\varepsilon$} \\
    $\{ (\tau.V)^*,\,\, \tau.J^c \} \gets$ \ID{$(\tau.S^c)^*$, $\varepsilon$} \\
    \reducelocalsamples{$R$, $\tau$}
  }
  \caption{Recursive HSS compression of a matrix $A$ with tolerance
    $\varepsilon$ for an HSS node $\tau$ using the random matrix $R$
    and the random samples $S^r$ and $S^c$.}
  \label{algo::HSScompressNode}
\end{algorithm}



==> tex/flop_count.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Flop Count

\clearpage

\subsection{Flop Count}

Here, we will be working through all of the details of the computational
cost of the flop count. The best case is $4mr^{2}$ in both situations,
although the worst case for doubling the number of samples is $16mr^{2}$.
The primary difference is the number of restarts required.
When adding $\del$ additional vectors each time, there are
asymptotically $\frac{r}{d}$ restarts, while only
$\log_{2}\parens{\frac{r}{d}}$ restarts when doubling the number of
samples at each step.

\subsubsection{$d$ Initial vectors; $\del$ additional vectors on restart}

Initially, we have $S = \begin{bmatrix} S_{0} & S_{1} \end{bmatrix}$,
where $S_{0}\in \R^{m\times d}$ and $S_{1}\in\R^{m\times \del}$
We compute $Q_{0} = \textbf{QR}(S_{0})$ ($2md^{2}$ flops)
and $S_{1} \equiv (I - Q_{0}Q_{0}^{*})S_{1}$ ($4md\del + m\del$ flops).
We now check to see if $||S_{1}||$ is small enough.
Here, we are using the $\del$ vectors to check the compression.

At step $n\ge1$, we have
$S = \begin{bmatrix} S_{0} & S_{1} & \cdots & S_{n} & S_{n+1} \end{bmatrix}$.
First, we compute $Q_{n} = \textbf{QR}(S_{n})$ ($2m\del^{2}$ flops).
Now, adding $Q_{n}$ to $Q$, the orthonormal basis vectors we have
already computed from the samples, we compute
$S_{n+1} \equiv (I - Q Q^{*})S_{n+1}$ ($4m(d + n\del)\del + m\del$ flops).
We will perform these computations
$N \sim \frac{r - d}{\del} \sim \frac{r}{\del}$ times, leading to
the flops

\begin{align}
F   &= 2md^{2} + 4md\del + m\del
        + \sum_{n=1}^{N}\brackets{2m\del^{2}
        + 4m\parens{d + n\del}\del + m\del}
        \nonumber\\
    &= 2md^{2} + 4(N+1)md\del + (N+1)m\del + 4m\del^{2}\sum_{n=1}^{N}n
        \nonumber\\
    &= 2md^{2} + 4(N+1)md\del + (N+1)m\del + 2m\del^{2}N(N+1)
        \nonumber\\
    &= 2md^{2} + 4\parens{\frac{r}{\del}+1}md\del
        + \parens{\frac{r}{\del}+1}m\del
        + 2m\del^{2}\parens{\frac{r}{\del}}\parens{\frac{r}{\del} + 1}
        \nonumber\\
    &\sim 2mr^{2}.
\end{align}

We see that this is the asymptotic result even if we use
$N \sim \frac{r}{\del} + 1$, which is the worst possible result:
we barely miss the rank of the underlying matrix whose range we
are trying to approximate. The RRQR cost is $2mr^{2}$, putting
the total cost at $4mr^{2}$ asymptotically, even in the worst case.

\subsubsection{$d$ Initial vectors; double each time}

We start with $S = \begin{bmatrix} S_{-1} & S_{0} \end{bmatrix}$,
where $S_{0} \in \R^{m\times d}$ and $S_{-1}\in\R^{m\times\ell}$.
Here $\ell$ is similar to the previous $\del$, as we will be using
the $\ell$ vectors of $S_{-1}$ to check the compression.
First, we compute $Q_{0} = \textbf{QR}(S_{0})$ ($2md^{2}$ flops)
and $S_{-1}\equiv \parens{I - Q_{0} Q_{0}^{*}}S_{-1}$
($4md\ell + m\ell$ flops). At this point, we want to check
to see if $||S_{-1}||$ is small enough.

At step $n\ge1$, we have have
$S = \begin{bmatrix} S_{-1} & S_{0} & \cdots & S_{n-1} & S_{n} \end{bmatrix}$.
Here, $\begin{bmatrix} S_{0} & \cdots & S_{n-1} \end{bmatrix}$ 
and $S_{n}$ have $2^{n-1}d$ columns. Given
$Q = \begin{bmatrix} Q_{0} & \cdots & Q_{n-1} \end{bmatrix}$, we compute
$S_{n}\equiv \parens{I - Q Q^{*}}S_{n}$ ($4^{n}md^{2} + 2^{n-1}md$ flops)
and $Q_{n} = \textbf{QR}(S_{n})$ ($\frac{1}{2}4^{n}md^{2}$ flops).
Finally, we compute $S\equiv\parens{I - Q_{n} Q_{n}^{*}}S$
($2^{n+1}md\ell + m\ell$ flops) before we check $||S||$.
We perform this computation $N \sim \log_{2}\parens{\frac{r}{d}}$ times,
leading to

\begin{align}
F   &= 2md^{2} + 4md\ell + m \ell
            + \sum_{n=1}^{N}\brackets{\frac{3}{2}4^{n}md^{2} + 2^{n-1}md
            + 2^{n+1}md\ell + m\ell}
        \nonumber\\
    &= \frac{1}{2}md^{2} + \frac{3}{2}md^{2}\sum_{n=0}^{N}4^{n}
            + \parens{1 + N}m\ell + 2md\ell + 2md\ell\sum_{n=0}^{1}2^{n}
            + md\sum_{n=0}^{N-1}2^{n}
        \nonumber\\
    &= \frac{1}{2}md^{2} + \frac{1}{2}md^{2}\brackets{4\cdot 4^{N} - 1}
        + \parens{1 + N}md\ell + 4\cdot2^{N}md\ell + \parens{2^{N} - 1}md
        \nonumber\\
    &\sim 2mr^{2}.
\end{align}

In the worst case, we have the total flops $\sim8mr^{2}$.
The RRQR cost is $2mr^{2}$ in the best case and $8mr^{2}$ in the
worst case, putting the total cost between $4mr^{2}$ and
$16mr^{2}$ asymptotically. The asymptotically worst case
will happen if we just miss the required rank, leading us
to use almost twice the necessary number of random vectors and
samples.

\clearpage


==> tex/power_method.tex <==
\subsection{Power-Method for Matrix-free Compression}

In this section, we discuss the possibility of using
a power iteration to speed up the convergence of HSS 
via randomized sampling.

